Individual qubit addressing of rotating ion crystals in a Penning trap

Trapped ions boast long coherence times and excellent gate fidelities, making them a useful platform for quantum information processing. Scaling to larger numbers of ion qubits in RF Paul traps demands great effort. Another technique for trapping ions is via a Penning trap where a 2D crystal of hundreds of ions is formed by controlling the rotation of the ions in the presence of a strong magnetic field. However, the rotation of the ion crystal makes single ion addressability a significant challenge. We propose a protocol that takes advantage of a deformable mirror to introduce AC Stark shift patterns that are static in the rotating frame of the crystal. Through numerical simulations we validate the potential of this protocol to perform high-fidelity single-ion gates in crystalline arrays of hundreds of ions.

==> old/todo.tex <==
\begin{enumerate}
    \item Make Ana's suggested changes to text.
    \item Figure for discussion about deformable mirror.
    \item Demonstrate that number of Zernike polynomials required for $r_1, r_2$. 
    \item Add in U, time, etc.
    \item Read through text again.
\end{enumerate}

==> old/todo_1.tex <==
1. John should be last author, since they're his ideas. \textbf{DONE}
2. Should Graeme be added since he's paying me?\textbf{DONE: He said no.}
3. Fig1. is already published, we might need to get rights to republish it.
4. Describe everything in figure 1.
5. Take my introduction in old.tex and put it before john's in main.tex \textbf{DONE}
6. Coloumb forces cannot couple the ions well, it would take longer than 10 seconds. Echacnage interactison, coloomb forces couple singlet to triplet states. Whewn e- are in diff orbtral singlet and triplets come into play, l=0, l=1, orbital and psin ? then put in colimn spin depp force. 
means direct need laser to couple with light
7. instead of normal 2d pictures, use trigangular lattice geometry.\textbf{DONE}
8. 1d plots for rqa (compare different rotation frequencies)\textbf{DONE}
9. Nonlinear regime just cnosdier two polynpmials in 2d plot
10. For a given # of ernike see how bad we are at reconstruction
for instance F of a fgate in a 2d trap fo n=5 and n=10
11. For the context of the paper might be better to resoncstruct, rather than just apply a gaussian.
12. Annulus is useful for pwave suiperconductors and geneartaion of majotrana modes. Resovling bands, maybe braiding.


13. ~100 ions is enough, 
